Differentially Private Graph Learning via Sensitivity-Bounded Personalized PageRank

Personalized PageRank (PPR) is a fundamental tool in unsupervised learning of graph representations such as node ranking, labeling, and graph embedding. However, while data privacy is one of the most important recent concerns, existing PPR algorithms are not designed to protect user privacy. PPR is highly sensitive to the input graph edges: the difference of only one edge may cause a big change in the PPR vector, potentially leaking private user data. In this work, we propose an algorithm which outputs an approximate PPR and has provably bounded sensitivity to input edges. In addition, we prove that our algorithm achieves similar accuracy to non-private algorithms when the input graph has large degrees. Our sensitivity-bounded PPR directly implies private algorithms for several tools of graph learning, such as, differentially private (DP) PPR ranking, DP node classification, and DP node embedding. To complement our theoretical analysis, we also empirically verify the practical performances of our algorithms.

==> data_final/blogcatalog-ndcg.tex <==
epsilon dpppr dpppr-prepush baseline
0.1 89.9210 95.0626 94.2973
0.5 96.2438 97.3319 97.8966
1.0 97.8403 98.3395 98.8714
2.0 98.7501 99.0360 99.3720
3.0 99.0564 99.2751 99.5370
4.0 99.1988 99.3970 99.6829
5.0 99.2727 99.4721 99.8461


==> data_final/blogcatalog-recall.tex <==
epsilon dpppr dpppr-prepush baseline
0.1 21.2487 64.9760 61.1450
0.5 69.7639 78.0853 79.2410
1.0 79.6027 82.1432 82.2290
2.0 81.1764 83.3071 83.4670
3.0 81.7409 83.4186 83.9400
4.0 81.7999 83.0839 85.3880
5.0 81.8511 83.4905 90.4880

==> data_final/pos-ndcg.tex <==
epsilon dpppr dpppr-prepush baseline
0.1 90.0519 96.0242 95.1975
0.5 95.5837 97.6606 97.9899
1.0 97.0556 98.3098 98.7357
2.0 98.1264 98.8938 99.2380
3.0 98.5423 99.1574 99.4493
4.0 98.7505 99.2992 99.6666
5.0 98.8706 99.3847 99.8550

==> data_final/pos-recall.tex <==
epsilon dpppr dpppr-prepush baseline
0.1 14.3547 63.9588 63.6172
0.5 40.2363 73.8101 77.5215
1.0 58.2293 81.9663 85.3557
2.0 69.1318 88.2373 89.3014
3.0 71.1083 89.6024 90.6284
4.0 71.6082 90.0664 92.3301
5.0 71.7979 90.2904 94.8612

==> figures/blogcatalog-ndcg.tex <==
epsilon dpppr dpppr-prepush baseline
0.1 89.9210 95.0626 94.2973
0.5 96.2438 97.3319 97.8966
1.0 97.8403 98.3395 98.8714
2.0 98.7501 99.0360 99.3720
3.0 99.0564 99.2751 99.5370
4.0 99.1988 99.3970 99.6829
5.0 99.2727 99.4721 99.8461


==> figures/blogcatalog-recall.tex <==
epsilon dpppr dpppr-prepush baseline
0.1 21.2487 64.9760 61.1450
0.5 69.7639 78.0853 79.2410
1.0 79.6027 82.1432 82.2290
2.0 81.1764 83.3071 83.4670
3.0 81.7409 83.4186 83.9400
4.0 81.7999 83.0839 85.3880
5.0 81.8511 83.4905 90.4880

==> figures/pos-ndcg.tex <==
epsilon dpppr dpppr-prepush baseline
0.1 90.0519 96.0242 95.1975
0.5 95.5837 97.6606 97.9899
1.0 97.0556 98.3098 98.7357
2.0 98.1264 98.8938 99.2380
3.0 98.5423 99.1574 99.4493
4.0 98.7505 99.2992 99.6666
5.0 98.8706 99.3847 99.8550

==> figures/pos-recall.tex <==
epsilon dpppr dpppr-prepush baseline
0.1 14.3547 63.9588 63.6172
0.5 40.2363 73.8101 77.5215
1.0 58.2293 81.9663 85.3557
2.0 69.1318 88.2373 89.3014
3.0 71.1083 89.6024 90.6284
4.0 71.6082 90.0664 92.3301
5.0 71.7979 90.2904 94.8612
